Guided Image-to-Image Translation with Bi-Directional Feature Transformation

We address the problem of guided image-to-image translation where we translate an input image into another while respecting the constraints provided by an external, user-provided guidance image. Various conditioning methods for leveraging the given guidance image have been explored, including input concatenation , feature concatenation, and conditional affine transformation of feature activations. All these conditioning mechanisms, however, are uni-directional, i.e., no information flow from the input image back to the guidance. To better utilize the constraints of the guidance image, we present a bi-directional feature transformation (bFT) scheme. We show that our bFT scheme outperforms other conditioning schemes and has comparable results to state-of-the-art methods on different tasks.

==> overview.tex <==
\section{Overview}
\label{sec:overview}

In a guided image to image translation task, an additional input guides the translation process by setting some constraints. In such problems the mostly used approach is to concatenate the additional guidance input to the input image.

\badour{I do not know what I should write in overview}

\input{figure/fig_overview}


